Reducing Idleness in Financial Cloud Services via Multi-objective Evolutionary Reinforcement Learning based Load Balancer

In recent years, various companies have started to shift their data services from traditional data centers to the cloud. One of the major motivations is to save on operational costs with the aid of cloud elasticity. This paper discusses an emerging need from financial services to reduce the incidence of idle servers retaining very few user connections, without disconnecting them from the server side. This paper considers this need as a bi-objective online load balancing problem. A neural network based scalable policy is designed to route user requests to varied numbers of servers for the required elasticity. An evolutionary multi-objective training framework is proposed to optimize the weights of the policy. Not only is the new objective of idleness is reduced by over 130% more than traditional industrial solutions, but the original load balancing objective itself is also slightly improved. Extensive simulations with both synthetic and real-world data help reveal the detailed applicability of the proposed method to the emergent problem of reducing idleness in financial services.

==> egbbl.tex <==
\begin{thebibliography}{99}

\bibitem{Elasticity}
Al-Dhuraibi Y, Paraiso F, Djarallah N, et~al. 
Elasticity in cloud computing: State of the art and research challenges. 
IEEE Transactions on Services Computing, 2018, 11(2): 430-447.

\bibitem{Qu2019Auto}
Qu C, Calheiros R N, Buyya R. 
Auto-scaling web applications in clouds: A taxonomy and survey.
ACM Computing Surveys, 2018, 51(4): 33.

\bibitem{Stoll2006Elec}
Stoll H~R.
Electronic trading in stock markets.
Journal of Economic Perspectives, 2006, 20(1): 153-174.

\bibitem{li2019cloud}
Li F.
Cloud-native database systems at alibaba: Opportunities and challenges.
Proceedings of the VLDB Endowment, 2019, 12(12): 2263-2272.

\bibitem{easley2011microstructure}
Easley D, De Prado M L, O’Hara M. 
The microstructure of the flash crash.
Journal of Portfolio Management, 2011, 37(2): 118-128.

\bibitem{shafiq2022load}
Shafiq D A, Jhanjhi N Z, Abdullah A.
Load balancing techniques in cloud computing environment: A review.
Journal of King Saud University-Computer and Information Sciences, 2022, 34(7): 3910-3933.

\bibitem{sajjan2017load}
Sajjan R S, Yashwantrao B R.
Load balancing and its algorithms in cloud computing: A survey.
International Journal of Computer Sciences and Engineering, 2017, 5(1): 95-100.

\bibitem{johora2022load}
Johora F T, Ahmed I, Shajal M A I, et al.
A load balancing strategy for reducing data loss risk on cloud using remodified throttled algorithm.
International Journal of Electrical and Computer Engineering, 2022, 12(3): 3217.

\bibitem{sim2003ant}
Sim K M, Sun W H. 
Ant colony optimization for routing and load-balancing: Survey and new directions.
IEEE Transactions on Systems, Man, and Cybernetics-Part A: Systems and Humans, 2003, 33(5): 560-572.

\bibitem{gures2022machine}
Gures E, Shayea I, Ergen M, et al.
Machine learning based load balancing algorithms in future heterogeneous networks: A survey.
IEEE Access, 2022. 10: 37689-37717.

\bibitem{farag2021congestion}
Farag H, Stefanovi{\v{c}} {\v{C}}.
Congestion-aware routing in dynamic IoT networks: A reinforcement learning approach.
IEEE Global Communications Conference, 2021: 1-6.

\bibitem{afzal2019load}
Afzal S, Kavitha G.
Load balancing in cloud computing-A hierarchical taxonomical classification.
Journal of Cloud Computing, 2019, 8(1): 22.

\bibitem{carrion2022kubernetes}
Carri{\'o}n C.
Kubernetes scheduling: Taxonomy, ongoing issues and challenges.
ACM Computing Surveys, 2022, 55(7): 1-37.

\bibitem{Kashani2023Load}
Kashani M H, Mahdipour E. 
Load balancing algorithms in fog computing: A systematic review.
IEEE Transactions on Services Computing, 2023, 16(2): 1505-1521.

\bibitem{trivella2016load}
Trivella A, Pisinger D.
The load-balanced multi-dimensional bin-packing problem.
Computers \& Operations Research, 2016, 74: 152-164.

\bibitem{Kumar2019issues}
Kumar P, Kumar R.
Issues and challenges of load balancing techniques in cloud computing: A survey.
ACM Computing Surveys, 2019, 51(6).

\bibitem{basu2019learn}
Basu D, Wang X, Hong Y, et al.
Learn-as-you-go with megh: Efficient live migration of virtual machines.
IEEE Transactions on Parallel and Distributed Systems, 2019, 30(8): 1786-1801.

\bibitem{zhu2022qos}
Zhu J, Yang R, Sun X, et al. 
Qos-aware co-scheduling for distributed long-running applications on shared clusters.
IEEE Transactions on Parallel and Distributed Systems, 2022, 33(12): 4818-4834.

\bibitem{zhang2023smaf}
Zhang S, Guo Y, Guo Z, et al.
SMAF: A secure and makespan-aware framework for executing serverless workflows.
Science China Information Sciences, 2023, 66(3): 139105.

\bibitem{wang2022solving}
Wang G G, Gao D, Pedrycz W.
Solving multiobjective fuzzy job-shop scheduling problem by a hybrid adaptive differential evolution algorithm.
IEEE Transactions on Industrial Informatics, 2022, 18(12): 8519-8528.

\bibitem{kandel2012enterprise}
Kandel S, Paepcke A, Hellerstein J M, et al. 
Enterprise data analysis and visualization: An interview study.
IEEE Transactions on Visualization and Computer Graphics, 2012, 18(12): 2917-2926.

\bibitem{salimans2017evolution}
Salimans T, Ho J, Chen X, et al. 
Evolution strategies as a scalable alternative to reinforcement learning.
arXiv preprint arXiv:1703.03864, 2017.

\bibitem{QIAN2023241}
Qian C, Liu D X, Feng C, et al.
\newblock Multi-objective evolutionary algorithms are generally good: Maximizing monotone submodular functions over sequences.
Theoretical Computer Science, 2023, 943: 241-266.

\bibitem{coello2020ind}
Falc\'{o}n-Cardona J~G, Coello C~A~C.
Indicator-based multi-objective evolutionary algorithms: A comprehensive survey.
ACM Computing Surveys, 2020, 53(2): 35.

\bibitem{chen2021interactive}
Chen L, Xin B, Chen J. 
Interactive multi-objective evolutionary algorithm based on decomposition and compression.
Science China Information Sciences, 2021, 64: 1-16.

\bibitem{deb2002a}
Deb K, Pratap A, Agarwal S, et al.
A fast and elitist multiobjective genetic algorithm: NSGA-II.
IEEE Transactions on Evolutionary Computation, 2002, 6(2): 182-197.

\bibitem{wang2021evolutionary}
Wang Y, Xue K, Qian C. 
Evolutionary diversity optimization with clustering-based selection for reinforcement learning.
Proceedings of International Conference on Learning Representations, 2022.
% \url{https://openreview.net/forum?id=74x5BXs4bWD}.

\bibitem{kaushik2018multi}
Kaushik R, Chatzilygeroudis K, Mouret J B.
Multi-objective model-based policy search for data-efficient learning with sparse rewards.
Proceedings of Conference on Robot Learning, 2018, 87: 839-855.

\bibitem{schulman2017proximal}
Schulman J, Wolski F, Dhariwal P, et al.
Proximal policy optimization algorithms.
arXiv preprint arXiv:1707.06347, 2017.

\bibitem{mao2019variance}
Mao H, Venkatakrishnan S B, Schwarzkopf M, et al.
Variance reduction for reinforcement learning in input-driven environments.
Proceedings of International Conference on Learning Representations, 2019.
% \url{https://openreview.net/forum?id=Hyg1G2AqtQ}.

\bibitem{arora2018understanding}
Arora R, Basu A, Mianjy P, et al.
Understanding deep neural networks with rectified linear units.
Proceedings of International Conference on Learning Representations, 2018.
% \url{https://openreview.net/forum?id=B1J_rgWRW}.

\bibitem{bian2021robustness}
Bian C, Qian C, Yu Y, et al.
On the robustness of median sampling in noisy evolutionary optimization.
Science China Information Sciences, 2021, 64: 1-13.


\end{thebibliography}
